Generalised Interpolation by Solving Recursion-Free Horn Clauses

In this paper we present InterHorn, a solver for recursion-free Horn clauses. The main application domain of InterHorn lies in solving interpolation problems arising in software verification. We show how a range of interpolation problems, including path, transition, nested, state/transition and well-founded interpolation can be handled directly by InterHorn. By detailing these interpolation problems and their Horn clause representations, we hope to encourage the emergence of a common back-end interpolation interface useful for diverse verification tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{Nikolaj Bj{\o}rner, Fabio Fioravanti, Andrey Rybalchenko, \\ Valerio Senni (Eds.): First Workshop on \\ Horn Clauses for Verification and Synthesis (HCVS 2014)\\
EPTCS 169, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.169.5}{10.4204/EPTCS.169.5}}

